Enhance Diffusion to Improve Robust Generalization

Deep neural networks are susceptible to human imperceptible adversarial perturbations. One of the strongest defense mechanisms is \emph{Adversarial Training} (AT). In this paper, we aim to address two predominant problems in AT. First, there is still little consensus on how to set hyperparameters with a performance guarantee for AT research, and customized settings impede a fair comparison between different model designs in AT research. Second, the robustly trained neural networks struggle to generalize well and suffer from tremendous overfitting. This paper focuses on the primary AT framework - Projected Gradient Descent Adversarial Training (PGD-AT). We approximate the dynamic of PGD-AT by a continuous-time Stochastic Differential Equation (SDE), and show that the diffusion term of this SDE determines the robust generalization. An immediate implication of this theoretical finding is that robust generalization is positively correlated with the ratio between learning rate and batch size. We further propose a novel approach, \emph{Diffusion Enhanced Adversarial Training} (DEAT), to manipulate the diffusion term to improve robust generalization with virtually no extra computational burden. We theoretically show that DEAT obtains a tighter generalization bound than PGD-AT. Our empirical investigation is extensive and firmly attests that DEAT universally outperforms PGD-AT by a significant margin.

==> subfiles/6-Related_Work.tex <==
\section{Related Work}
\label{related_work}
% \vspace{-0.05in}

We summarize the related works in (A) Adversarial Training; (B) SDE Modeling of Stochastic Algorithms; and (C) Generalization and Hyperparameters in this section.

% \vspace{-0.05in}
\subsection{Adversarial Training}

Deep learning models have been widely applied in many different domains, e.g. \cite{Mnih2013PlayingAW,He2016DeepResNet,Devlin2019BERT,Jure2017GNN,google16deep&wide,SuoICHI19,Xun2020CorrelationNF,Zhou21WWW,DingZhou21WWW,Wei23ICML}, while they are observed to be susceptible to human imperceptible adversarial attacks \cite{Szegedy2014IntriguingPO,Goodfellow2015ExplainingAH,nguyen2015adversarial,zugner18adversarialgraph,Huai20attack,Sinha2022UnderstandingAE}. We refer readers to a comprehensive overview of adversarial attacks and defenses and references therein \cite{Chakraborty2018AdversarialAA}. An incomplete list of recent advances would include \cite{tramer2018ensemble, Zhang2019TheoreticallyPT, pmlr-v97-wang19i, Qin2019AdversarialRT, wang2018a, Mao2019MetricLF, Carmon2019UnlabeledDI, hendrycks2019pretraining, wu22adversarial,Wu2022AdversarialWP, Shafahi2019AdversarialTF, zhang2019you, Wong2020Fast}. This study focuses on PGD-AT \cite{madry2018towards}, the most commonly used adversarial training strategy, and we view PGD-AT as a minimax optimization problem \cite{lin20minimaxa,lin20minimaxb}, where the inner maximization optimizes an adversary while the outer minimization robustifies the model parameters.

% generates adversarial examples against the neural network via multi-step projected gradient descent, while in the outer minimization, the neural network is updated via a single-step gradient descent based on the generated perturbed data. Please refer to Section \ref{backgroun_section} for formal definition.


\subsection{SDE Modeling of Stochastic Algorithms}

\cite{Li17SME,Mandt17SGDApproximateBayesian} are the first works that approximate discrete-time stochastic gradient descent by continuous-time SDE. \cite{Krichene17Mirror,An2018StochasticME,Gitman19Momentum,Cao2020ApproximationAC} extended SDE modeling to accelerated mirror descent, asynchronous SGD, momentum SGD, and generative adversarial networks, respectively. \cite{liu2021noise} studied the SDE approximation of SGD with a moderately large learning rate, while approximation in \cite{Mandt17SGDApproximateBayesian} works best with infinitesimal step size. \cite{Chaudhari2017DeepRP,xie2021positive} designed an entropy regularization and a noise injection method, respectively, motivated by the SDE characterization of SGD. \cite{Gu2021AT_SDE} attempted to model adversarial training dynamics via SDE, while did not recognize the connection between dynamics and generalization error.

\subsection{Generalization and Stochastic Noise}

One of the goals of this paper is to theoretically and empirically study how stochastic noise impacts generalization in adversarial training. The research is mainly divided into two lines, the impact of hyperparameters on noise and directly injection of external noise. 

Existing works on hyperparameters are mainly on non-adversarial training, e.g., many recent works empirically report the influence of hyperparameters in SGD, largely on $b$ and $\alpha$, and provide practical tuning guidelines. \cite{Keskar16Large-Batch} empirically showed that the large-batch training leads to sharp local minima which has poor generalization, while small-batches lead to flat minima which makes SGD generalize well. \cite{GoyalDGNWKTJH17LargeMinibatch,jastrzebski2018three} proposed the Linear Scaling Rule for adjusting $\alpha$ as a function of $b$ to maintain the generalization ability of SGD. \cite{Smith18Bayesian,Smith18DontDecay} suggested that increasing $b$ during the training can achieve similar result of decaying the learning rate $\alpha$. 

Our generalization analysis relies on PAC-Bayesian inequalities \cite{Williamson97PAC-Bayes,McAllester98PAC-Bayes,Guedj2019APO}. \cite{London2017APA,He19ControlBatch,Sun21KDDHyperparameter,Sun22KDDHyper,Sun2023TKDD} proved a PAC-Bayesian bound for vanilla SGD, SGD with momentum, asynchronous SGD, all in a benign environment. 

The first and only systematic study on hyperparameters of adversarial training is \cite{pang2021bag}, to our best knowledge. The authors carefully evaluated a wide range of training tricks, including early stopping, learning rate schedule, activation function, model architecture, optimizer and many others. However, their findings do not provide theoretical insights why certain tricks work or fail. Our study aims to bridge this gap and motivate our novel training algorithm through theoretical findings.
